ConVer-G: Concurrent versioning of knowledge graphs

The multiplication of platforms offering open data has facilitated access to information that can be used for research, innovation, and decision-making. Providing transparency and availability, open data is regularly updated, allowing us to observe their evolution over time. We are particularly interested in the evolution of urban data that allows stakeholders to better understand dynamics and propose solutions to improve the quality of life of citizens. In this context, we are interested in the management of evolving data, especially urban data and the ability to query these data across the available versions. In order to have the ability to understand our urban heritage and propose new scenarios, we must be able to search for knowledge through concurrent versions of urban knowledge graphs. In this work, we present the ConVer-G (Concurrent Versioning of knowledge Graphs) system for storage and querying through multiple concurrent versions of graphs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=project

PDF = $(PACKAGE).pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

all:  ${PDF}

%.pdf: %.tex
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex -synctex=1 -interaction=nonstopmode -file-line-error $<; done

%.cls:   %.ins %.dtx
	pdflatex $<

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	./**/*.log ./**/*.aux \
	./**/*.cfg ./**/*.glo ./**/*.idx ./**/*.toc \
	./**/*.ilg ./**/*.ind ./**/*.out ./**/*.lof \
	./**/*.lot ./**/*.bbl ./**/*.blg ./**/*.gls ./**/*.cut ./**/*.hd \
	./**/*.dvi ./**/*.ps ./**/*.thm ./**/*.tgz ./**/*.zip ./**/*.rpi

clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE).synctex.gz

distclean: clean
	$(RM)  *.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip: 
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

.PHONY: all docclean clean distclean archive zip

